Managing O-RAN Networks: xApp Development from Zero to Hero

The Open Radio Access Network (O-RAN) Alliance proposes an open architecture that disaggregates the RAN and supports executing custom control logic in near-real time from third-party applications, the xApps. Despite O-RAN's efforts, the creation of xApps remains a complex and time-consuming endeavor, aggravated by the sometimes fragmented, outdated, or deprecated documentation from the O-RAN Software Community (OSC). These challenges hinder academia and industry from developing and validating solutions and algorithms on O-RAN networks. This tutorial addresses this gap by providing the first comprehensive guide for developing xApps to manage the O-RAN ecosystem from theory to practice. We provide a thorough theoretical foundation of the O-RAN architecture and detail the functionality offered by Near Real-Time RAN Intelligent Controller (Near-RT RIC) components. We examine the xApp design and configuration. We explore the xApp lifecycle and demonstrate how to deploy and manage xApps on a Near-RT RIC. We address the xApps' interfaces and capabilities, accompanied by practical examples. We provide comprehensive details on how xApps can control the RAN. We discuss debugging strategies and good practices to aid the xApp developers in testing their xApps. Finally, we review the current landscape and open challenges for creating xApps.

==> acronyms.tex <==
% !TEX root = ../main.tex
%\section*{DeclareAcronymnyms}

% \begin{DeclareAcronymnym}[IMT-Advanced]

\DeclareAcronym{3GPP}{
    short=3GPP,
    long=3rd Generation Partnership Project
}

\DeclareAcronym{RAN}{
    short = {RAN},
    long  = {Radio Access Network},
}

\DeclareAcronym{UE}{
    short = {UE},
    long  = {User Equipment},
}

\DeclareAcronym{MEC}{
    short = {MEC},
    long  = {Multi-access Edge Computing},
}

\DeclareAcronym{MEID}{
    short = {MEID},
    long  = {Managed Entity ID},
}

\DeclareAcronym{AI}{
    short = {AI},
    long  = {Artificial Intelligence},
}


\DeclareAcronym{COTS}{
    short = {COTS},
    long  = {Commercial Off-The-Shelf},
}

\DeclareAcronym{DSP}{
    short = {DSP},
    long  = {Digital Signal Processor},
}

\DeclareAcronym{FPGA}{
    short = {FPGA},
    long  = {Field Programmable Gate Array},
}

\DeclareAcronym{ML}{
    short = {ML},
    long  = {Machine Learning},
}

\DeclareAcronym{O-RAN}{
    short = {O-RAN},
    long  = {\acl{O} \acl{RAN}},
}

\DeclareAcronym{nearrtric}{
    short = {Near-RT RIC},
    long  = {Near Real-Time \acl{RIC}},
}

\DeclareAcronym{SMO}{
    short = {SMO},
    long  = {Service Management and Orchestration},
}

\DeclareAcronym{nonrtric}{
    short = {Non-RT RIC},
    long  = {Non Real-Time \acl{RIC}},
}

\DeclareAcronym{SDR}{
    short = {SDR},
    long  = {Software Defined Radio},
}

\DeclareAcronym{RU}{
    short = {RU},
    long  = {Radio Unit},
}

\DeclareAcronym{DU}{
    short = {DU},
    long  = {Distributed Unit},
}

\DeclareAcronym{CU}{
    short = {CU},
    long  = {Centralized Unit},
}


\DeclareAcronym{ORU}{
    short = {O-RU},
    long  = {\ac{O}\ac{RU}},
}

\DeclareAcronym{ODU}{
    short = {O-DU},
    long  = {\ac{O}\ac{DU}},
}

\DeclareAcronym{OCU}{
    short = {O-CU},
    long  = {\ac{O}\ac{CU}},
}

\DeclareAcronym{OSC}{
    short = {OSC},
    long  = {\acs{O-RAN} Software Community},
}

\DeclareAcronym{RRU}{
    short = {RRU},
    long  = {Remote Radio Unit},
}


\DeclareAcronym{BBU}{
    short = {BBU},
    long  = {Base Band Unit},
}

\DeclareAcronym{ONF}{
    short = {ONF},
    long  = {Open Networking Foundation},
}

\DeclareAcronym{RIC}{
    short = {RIC},
    long  = {\ac{RAN} Intelligent Controller},
}

\DeclareAcronym{SM}{
    short = {SM},
    long  = {Service Model},
}

\DeclareAcronym{RC}{
    short = {RC},
    long  = {\ac{RAN} Control},
}

\DeclareAcronym{CCC}{
    short = {CCC},
    long  = {Cell Configuration and Control},
}

\DeclareAcronym{E2SM}{
    short = {E2SM},
    long  = {E2 \ac{SM}},
}

\DeclareAcronym{E2AP}{
    short = {E2AP},
    long  = {E2 Application Protocol},
}

\DeclareAcronym{NIB}{
    short = {NIB},
    long  = {Network Information Base},
}

\DeclareAcronym{IE}{
    short = {IE},
    long  = {Information Element},
}

\DeclareAcronym{AIMLFW}{
    short = {AIMLFW},
    long  = {AI/ML Framework}
}

\DeclareAcronym{UENIB}{
    short = {UE-NIB},
    long  = {\acl{UE}-\ac{NIB}},
}

\DeclareAcronym{RNIB}{
    short = {R-NIB},
    long  = {Radio-\ac{NIB}},
}

\DeclareAcronym{PRB}{
    short = {PRB},
    long  = {Physical Resource Block},
}

\DeclareAcronym{QoS}{
    short = {QoS},
    long  = {Quality of Service},
}

\DeclareAcronym{QoE}{
    short = {QoE},
    long  = {Quality of Experience},
}

\DeclareAcronym{QCI}{
    short = {QCI},
    long  = {Class Identifier},
}

\DeclareAcronym{OID}{
    short = {OID},
    long  = {Object Identifier},
}

\DeclareAcronym{LTE}{
    short = {LTE},
    long  = {Long-Term Evolution},
}

\DeclareAcronym{CN}{
    short = {CN},
    long  = {Core Network},
}

\DeclareAcronym{EPC}{
    short = {EPC},
    long  = {Evolved Packet Core},
}

\DeclareAcronym{IQ}{
    short = {IQ},
    long  = {In-phase/Quadrature},
}

\DeclareAcronym{UHD}{
    short = {UHD},
    long  = {USRP Hardware Driver},
}


\DeclareAcronym{UPF}{
    short = {UPF},
    long  = {User Plane Function},
}

\DeclareAcronym{UP}{
    short = {UP},
    long  = {User Plane},
}

\DeclareAcronym{RAT}{
    short = {RAT},
    long  = {Radio Access Technology},
}


\DeclareAcronym{OSM}{
    short = {OSM},
    long  = {Open Source MANO},
    % ewb: I took out MANO - it did not expand well and is itself an acronym and was used only once in the paper.
}

\DeclareAcronym{ONAP}{
    short = {ONAP},
    long  = {Open Networking Automation Platform},
}


\DeclareAcronym{MAC}{
    short = {MAC},
    long  = {Medium Access Control},
}

\DeclareAcronym{PHY}{
    short = {PHY},
    long  = {Physical},
}

\DeclareAcronym{CP}{
    short = {CP},
    long  = {Control Plane},
}

\DeclareAcronym{O}{
    short = {O-},
    long  = {Open},
    class = test
}

\DeclareAcronym{RF}{
    short = {RF},
    long  = {Radio Frequency},
}

\DeclareAcronym{S1AP}{
    short = {S1AP},
    long  = {S1 Application Protocol},
}

\DeclareAcronym{REST}{
    short = {REST},
    long  = {Representational State Transfer},
}

\DeclareAcronym{CCI}{
    short = {CCI},
    long  = {Commonwealth Cyber Initiative},
}

\DeclareAcronym{C-RAN}{
    short = {C-RAN},
    long  = {Cloud \ac{RAN}},
}

\DeclareAcronym{KPI}{
    short={KPI},
    long={Key Performance Indicator}
}

\DeclareAcronym{KPM}{
    short={KPM},
    long={Key Performance Measurement}
}

\DeclareAcronym{SLA}{
  short={SLA},
  long={Service Level Agreement}
}

\DeclareAcronym{MNO}{
    short=MNO,
    long=Mobile Network Operator
}

\DeclareAcronym{OC}{
    short={O-Cloud},
    long={\acl{O} Cloud}
}

\DeclareAcronym{PDCP}{
    short={PDCP},
    long={Packet Data Convergence Protocol}
}

\DeclareAcronym{SDAP}{
    short={SDAP},
    long={Service Data Adaptation Protocol}
}

\DeclareAcronym{RRC}{
    short={RRC},
    long={Radio Resource Control}
}

\DeclareAcronym{FCAPS}{
    short={FCAPS},
    long={Fault,\;Configuration,\;Accounting, Performance, and Security}
}

\DeclareAcronym{eMBB}{
    short={eMBB},
    long={enhanced Mobile Broadband}
}

\DeclareAcronym{mMTC}{
    short={mMTC},
    long={massive Machine Type Communications}
}

\DeclareAcronym{URLLC}{
    short={URLLC},
    long={Ultra Reliable Low Latency Communications}
}

\DeclareAcronym{FFT}{
    short={FFT},
    long={Fast Fourier Transform}
}

\DeclareAcronym{IFFT}{
    short={IFFT},
    long={Inverse FFT}
}

\DeclareAcronym{SDN}{
    short={SDN},
    long={Software-Defined Networking}
}

\DeclareAcronym{SDL}{
    short={SDL},
    long={Shared Data Layer}
}

\DeclareAcronym{STSL}{
    short={STSL},
    long={Shared Time Series Layer}
}

\DeclareAcronym{RMR}{
    short={RMR},
    long={\ac{RIC} Message Router}
}

\DeclareAcronym{OAI}{
    short={OAI},
    long={OpenAirInterface}
}

\DeclareAcronym{AAA}{
    short={AAA},
    long={Authentication,\;Authorization,\;and Accountability}
}

\DeclareAcronym{srsLTE}{
    short={srsLTE},
    long={Software Radio Systems Long Term Evolution}
}

\DeclareAcronym{DRL}{
    short={DRL},
    long={Deep Reinforcement Learning}
}

\DeclareAcronym{GNN}{
    short={GNN},
    long={Graph Neural Network}
}


\DeclareAcronym{DMS}{
    short={DMS},
    long={Deployment Management Service}
}

\DeclareAcronym{CLI}{
    short={CLI},
    long={Command Line Interface}
}

\DeclareAcronym{VES}{
    short={VES},
    long={Virtual Event Streaming}
}

\DeclareAcronym{VESPA}{
    short={VESPA},
    long={\ac{VES} Prometheus Adapter}
}

\DeclareAcronym{PLMN}{
    short={PLMN},
    long={Public Land Mobile Network}
}

\DeclareAcronym{AC}{
    short={AC},
    long={Admission Control}
}

\DeclareAcronym{TS}{
    short={TS},
    long={Traffic Steering}
}

\DeclareAcronym{AD}{
    short={AD},
    long={Anomaly Detection}
}

\DeclareAcronym{MLB}{
    short={MLB},
    long={Mobility Load Balancing}
}

\DeclareAcronym{RSM}{
    short={RSM},
    long={RAN Slice Manager}
}

\DeclareAcronym{MHO}{
    short={MHO},
    long={Mobile Handover}
}

